Specifying and Verifying Properties of Space - Extended Version

The interplay between process behaviour and spatial aspects of computation has become more and more relevant in Computer Science, especially in the field of collective adaptive systems, but also, more generally, when dealing with systems distributed in physical space. Traditional verification techniques are well suited to analyse the temporal evolution of programs; properties of space are typically not explicitly taken into account. We propose a methodology to verify properties depending upon physical space. We define an appropriate logic, stemming from the tradition of topological interpretations of modal logics, dating back to earlier logicians such as Tarski, where modalities describe neighbourhood. We lift the topological definitions to a more general setting, also encompassing discrete, graph-based structures. We further extend the framework with a spatial until operator, and define an efficient model checking procedure, implemented in a proof-of-concept tool.

==> boundaries.tex <==
\section{Boundaries}

In \cite{Gal99}, a discrete variant of the topological definition of the boundary of a set $A$ is given, for the case where a closure operator is derived by \autoref{def:closure-operator-of-a-relation} from a reflexive and symmetric relation. Therein, in Lemma 5, it is proved that the definition coincides with the one we provide below. The latter is only given in terms of closure and interior, and coincides with the definition of boundary in a topological space. We shall also make use of two variants on this notion, namely the \emph{interior} and \emph{closure} boundaries.

\begin{definition}\label{def:boundary}
 In a closure space $(X,\closure)$, the \emph{boundary} of $A \subseteq X$ is defined as $\boundary(A) = \closure(A) \setminus \interior(A)$. The \emph{interior boundary} is $\iboundary(A) = A \setminus \interior(A)$, and the \emph{closure boundary} is $\cboundary(A) = \closure(A) \setminus A$.
\end{definition}

\begin{proposition}\label{pro:boundary-properties}
 The following equations hold in a closure space:

 \begin{align}
    \boundary(A) & =  \cboundary(A) \cup \iboundary(A)  \label{eqn:boundary-properties-1}\\
    \cboundary(A) \cap \iboundary(A) & = \emptyset \label{eqn:boundary-properties-2} \\
    \boundary(A) & =  \boundary(\overline A) \label{eqn:boundary-properties-3} \\
    \cboundary(A) & =  \iboundary(\overline A)  \label{eqn:boundary-properties-4} \\
    \cboundary(A) & =  \boundary(A) \cap \overline A \label{eqn:boundary-properties-5} \\
    \iboundary(A) & =  \boundary(A) \cap A \label{eqn:boundary-properties-6} \\
    \boundary(A) & =  \closure(A) \cap \closure(\overline A) \label{eqn:boundary-properties-7}
 \end{align}
\end{proposition}

% % % \section{Continuous functions and observability}
% % % \begin{todo}
% % %  This section is provisional.
% % % \end{todo}
% % % 
% % % In this section we establish the relationship between logical equivalence under $\dsl$ formulae and identifiability under morphisms. For this, we shall establish a notion of morphism of model. In the following, for $A \subseteq X$ and $f : X \to Y$, let us use the shorthand $f(A) = \{ f(x) \mid x \in A \}$.
% % % 
% % % \begin{definition}
% % %  Given closure spaces $(X,\closure_X)$, $(Y,\closure_Y)$, a function $f : X \to Y$ is called \emph{continuous} whenever, for all $A \subseteq X$, it holds that $f(\closure_X(A)) \subseteq \closure_Y(f(A))$. In this case, we also write $f : (X, \closure_X) \to (Y, \closure_Y)$ to denote that $f : X \to Y$ is continuous.
% % % \end{definition}
% % % 
% % % \begin{definition}
% % % Assume a fixed set $\props$ of proposition letters, and consider models $\model_X = ((X, \closure_X), \eval_X)$, $\model_Y = ((Y, \closure_Y), \eval_Y)$. Call a continuous function $f : (X, \closure_X) \to (Y, \closure_Y)$ a \emph{continuous model homomorphism}, or simply a \emph{homomorphism}, whenever, for all $x \in X$, and $p \in \props$, it holds that $x \in \eval_X(p) \iff f(x) \in \eval_Y(p)$. In words, it is required that $f$ preserves and reflects the valuation of propositions at points. We write $f : \model_X \to \model_Y$ to signify that $f$ is a homomorphism.
% % % \end{definition}

% First, we establish a correctness result for $\dsl$: when points are distinguished by some formula, they can not be equated by morphisms.
% 
% \begin{proposition}
%  Morphisms preserve formulas: for all $\phi$, $\model = ((X,\closure),\eval)$, $x \in X$, $\model'$, $f : \model \to \model'$, we have $\model, x \models \phi \implies \model', f(x) \models \phi$.
% \end{proposition}
% 
% \begin{proof}
%  By induction on the structure of $\phi$. We omit the trival case when $\phi = \top$, and the cases for the operators $\lnot$ and $\land$, which are just an application of the induction hypothesis.
%  
%  \begin{description}
%     \item[Case $\phi = p$:]
%     $\der 
%     \model, x \models \phi 
%     \stp \iff x \in \eval(p) 
%     \jstp \implies {f $ is a homomorphism$} f(x) \in \eval(p)
%     \stp \iff f(x) \models \phi$
% 
%     \item[Case $\phi = \psi \until \xi$:]
%     $\der
%     \model, x \models \psi \until \xi$
%   \end{description}
% \end{proof}
% 
% 
% \begin{proposition}
%  Let $\model = ((X,\closure),\eval$. For $x,y \in X$, whenever there is a $\dsl$ formula $\phi$ such that $\model, x \models \phi$ and $\model, y \nmodels \phi$, there is no model $\model'$ and morphism $f : \model \to \model'$ such that $f(x) = f(y)$.
% \end{proposition}

% \section{Outside and inside of a curve}
% 
% \begin{todo}
%  This section is provisional. More precise statements and references should be provided.
% \end{todo}
% 
% A problem affects the definition of $\until$ even in topological spaces. It is not possible to tell apart points that are inside of a digital curve from points that are outside. Consider a black circle on a white background in $\reals^2$, that is the set $\{ (x,y) \mid x^2 + y^2 = 1 \}$. The points inside the circle satisfy $white \until black$, but also the points outside of it satisfy it; to see this, chose the open set $\{ (x,y) \mid x^2 + y^2 > 1 \}$. However, it is possible in topology to tell apart the two regions of the plane corresponding to the inside and the outside of a closed curve in the digital plane.
% 
% First, one looks at Jordan's curve theorem, whose proof is considered to be very hard in mathematics. 
% 
% \begin{definition}
% A \emph{simple closed curve} is the image of an injective continuous function from the topological space $U$ of the unit circle (that is, the subspace topology over the set $\{ (x,y) \mid x^2 + y^2 = 1\} \subseteq \reals^2)$.
%  \end{definition}
% 
% \begin{proposition}\label{pro:jordan-theorem}
%  A simple closed curve separates the plane in two connected components. 
% \end{proposition}
% 
% The theorem states that the two regions that we are interested in are connected, but it does not say what is the inside and what is the outside. For this, one uses homotopy. We would like to characterise the inner region as the place $R$ where all closed curves can be continuously deformed to a point, in such a way that all the steps of the deformation lie in $R$. The formalisation of this requires the concept of homotopy.
% 
% \begin{definition}
%  Fix two topological spaces $S_X = (X,\open_X)$ and $S_Y = (Y,\open_Y)$, and the space $[0,1]\subseteq \reals$ equipped with the subspace topology. Consider two continuous functions $f,g : S_X \to S_Y$. An \emph{homotopy} $h$ from $f$ to $g$, written $h : f \to g$, is a continuous function $h : S_X \times [0,1] \to S_Y$ such that, for all $x \in X$, $h(x,0) = f(x)$, and for all $y \in Y$, $h(y,0) = g(x)$. 
% \end{definition}
% 
% In words, $h$ is a ``continuous deformation'' from $f$ to $g$, turning $f$ into $g$ in continuous steps over the object of time $[0,1]$. Once established this, we can define the inner region of a simple closed curve. 
% 
% \begin{definition}
%  A path-connected subset $R$ of a topological space $S$ is called \emph{simply connected} whenever, for each closed curve $f : U \to S$ whose image lies in $R$, there is a point $y$ and a constant closed curve $g : U \to S$, with $g(x) = y$ for all $x$, and a homotopy $h : f \to g$ such that, for all $t \in [0,1]$, and $x$, we have $h(x,t) \in R$.  
% \end{definition}
% 
% In the plane, Jordan's theorem can be improved by saying that a simple closed curve separates the plane in two connected components (Q: connected or path-connected, what is really relevant for the definition of simple connectedness?), and just one of them is simply connected. In a sphere, this is not possible.
% 
% We now look at the situation in graphs. We need to define a ``plane-alike'' graph and a ``sphere-alike'' graph. Consider the graph associated to the vertexes and edges of a cube with four added vertices, dividing in two parts four parallel edges, and four added edges defining a closed curve that cuts the cube into two parts. Then both sides of the curve would be ``simply connected'', whatever the definition of homotopy over discrete structures is. One may expect that the concept of planarity helps, but this is not the case. There are two planar layouts of the mentioned graph, that are isomorphic, one of them keeping a different face of the cube inside (ask Vincenzo for details).
% 
% A simple fix to the situation is to invent a restricted kind of closure spaces, called \emph{bounded closure spaces}.
% 
% \begin{definition}
%  A \emph{bounded} closure space is a structure $(X,\closure,\eow)$ where $(X,\closure)$ is a closure space, and $\eow \subseteq X$ is a set of points called \emph{bounding set} or \emph{end of world predicate} of the space.
% \end{definition}
% 
% We assume the natural extension of concepts such as quasi-discreteness, closure models, satisfaction of $\dsl$ formulae, and so on, to be extended to bounded closure spaces, so that we can speak, e.g., of a quasi-discrete bounded closure space, or a bounded (closure) model.
% 
% \begin{note}
%  V: I am not putting constraints on what the bounding box is, at the moment. If it comes handy in proofs, or if it is more pleasing to us, we could impose that $\eow$ is a closed curve, to be defined, very likely just as in topological spaces (I know more about this, we can discuss the situation). Additionally, we could require that the whole space is non-empty, connected, and so is the space minus the bounding set is also connected. Thus, the boundary would be a very special kind of ``Jordan curve in a closure space'' (this concept is still undefined in my opinion), which separates the plane into two connected components, one empty and one non-empty, thus making the distinction between the inside and outside of the bounding set trivial by construction.
% \end{note}
% 
% Using bounded closure spaces, we can provide stricter versions of the until operator.
% 
% \begin{definition}\label{def:inside-operator}
%  We define the binary logical operator \emph{surrounded by}, written $\inside$. The semantics of the operator is defined on a bounded model $\model = ((X,\closure,\eow),\eval)$ at point $x \in X$ as follows:
%  \[\begin{array}{rcl}
%    \model,x \models \phi \inside \psi & \iff & \exists A \subseteq X . \closure(\interior(A))=A \land x \in \interior(A) \land \\ & & \qquad \land \forall y \in \interior(A) . (y \notin \eow \land \model, y \models \phi) \land \\ & & \qquad \land \forall z \in \iboundary(A) . \model, z \models \psi
%  \end{array}\]
% \end{definition}
% 
% Next, we provide a characterising theorem for the $\inside$ operator. For this, we need the notion of \emph{path}. 
% 
% \begin{definition}\label{def:path}
%  In a closure space $(X,\closure)$, a \emph{path} from $x \in X$ to $y \in X$ is a continuous function from the subspace generated by $[0,1]$ of the Euclidean topology on $\reals$ to $(X,\closure)$, such that $f(0)=x$ and $f(1)=y$.
% \end{definition}
% 
% \begin{todo}
%  V: A digression here is needed to discuss what are paths in a quasi-discrete closure space. From \cite{Gal03} it seems like only finite paths are required in that case, the whole issue is a bit fuzzy to me at the moment.
% \end{todo}
% 
% \begin{theorem}\label{thm:until-implies-path}
%  Whenever $\model, x \models \phi \inside \psi$, then for all points $y \in \eow$ and all paths $f$ from $x$ to $y$, there is $t \in [0,1]$ such that $\model, f(t) \models \psi$.
% \end{theorem}
% 
% \begin{proof}(of \autoref{thm:until-implies-path})
%   Recall that in $\reals$ equipped with the Euclidean topology, we have $k \in \closure(A) \iff \exists \epsilon . \forall k' \in (k, k+\epsilon) . k' \in A \lor \forall k'' \in (k-\epsilon, k) . k'' \in A$. As a corollary, the least upper bound and greatest lower bound of a set belong to its closure. (TODO).
%   %
%   Consider the set $S_- = \{ k \in [0,1] \mid \forall k' \in [0,k] . f(k') \in \interior(A) \}$, and the set $S_+ = \{ k \in [0,1] \mid \exists k' \in [0,k] . f(k') \in \overline{\interior(A)} = \closure(\overline A) \}$. 
%   %
%   Notice that $S_{-}$ and $S_+$ are nonempty (they contain $0$, and $1$, respectively) and that they are bounded by $[0,1]$, thus they admit least upper bound and greatest lower bound. Let $k_-$ be the least upper bound of $S_-$ and $k_+$ be the greatest lower bound of $S_+$. 
%   Moreover (TODO) $k_+$ is an upper bound of $S_-$ and $k_-$ is a lower bound of $S_+$, therefore $k_- \leq k_+$.
%   %
%   We first conclude the proof in the case $k_- = k_+$. 
%   %
%   Since $k_- \in \closure(S_-)$, we have $f(k_-) \in \closure(f(S_-))$, but also $f(S_-) \subseteq \interior(A)$;  by monotonicity of closure, we note that $f(k_-) \in \closure(\interior(A)) = A$. 
%   %
%   %On the other hand, $k$ is also the greatest lower bound of $\{ k \mid f(k) \in \overline A \}$ (TODO). Thus by continuity we need $k \in \closure(\overline A)$. By this, $k \in A \cap \closure(\overline(A)) = A \cap \overline{\interior(A)} = A \setminus \interior(A) = \iboundary(A)$.
%   %
%   %If $k_- < k_+$, consider a point $k_0 \in (k_-,k_+)$. We have that $k_0$ is a upper bound of $S_-$, and not the least one, so it belongs to the complement of $S_-$. Similarly, $k_0$ also belongs to the complement of $S_+$. Therefore there is $k' \leq k_0$ with 
%   %$f(k') \in \interior(A)$, and for all $k'' \leq k$ we have $f(k'') \notin \overline A$. Therefore, $f(k')$ must belong to $A \setminus \interior(A) = \iboundary(A)$.
% \end{proof}

% \begin{proof}(of \autoref{thm:until-implies-path})
%   Recall that in $\reals$ equipped with the Euclidean topology, we have $k \in \closure(A) \iff \exists \epsilon . \forall k' \in (k, k+\epsilon) . k' \in A \lor \forall k'' \in (k-\epsilon, k) . k'' \in A$. As a corollary, the least upper bound and greatest lower bound of a set belong to its closure. (TODO).
%   %
%   Consider the set $S_- = \{ k \in [0,1] \mid \forall k' \in [0,k] . f(k') \in \interior(A) \}$, and the set $S_+ = \{ k \in [0,1] \mid \exists k' \in [0,1] . k' \leq k \land f(k') \in \overline A \}$. 
%   %
%   Notice that $S_{-}$ and $S_+$ are nonempty and bounded; by this, let $k_-$ be the least upper bound of $S_-$ and $k_+$ be the greatest lower bound of $S_+$. Notice that $S_-$ is downward closed and $S_+$ is upward closed; 
%   %
%   by this, $k_+$ is an upper bound of $S_-$ and $k_-$ is a lower bound of $S_+$, therefore $k_- \leq k_+$. We first continue the proof in the case $k=k_- = k_+$. Notice $f(S_-) \subseteq \interior(A)$; since $k \in \closure(S_-)$, and by monotonicity of closure, we have $k \in \closure(\interior(A)) = A$. 
%   %
%   On the other hand, $k$ is also the greatest lower bound of $\{ k \mid f(k) \in \overline A \}$ (TODO). Thus by continuity we need $k \in \closure(\overline A)$. By this, $k \in A \cap \closure(\overline(A)) = A \cap \overline{\interior(A)} = A \setminus \interior(A) = \iboundary(A)$.
%   %
%   If $k_- < k_+$, consider a point $k_0 \in (k_-,k_+)$. We have that $k_0$ is a upper bound of $S_-$, and not the least one, so it belongs to the complement of $S_-$. Similarly, $k_0$ also belongs to the complement of $S_+$. Therefore there is $k' \leq k_0$ with 
%   $f(k') \in \interior(A)$, and for all $k'' \leq k$ we have $f(k'') \notin \overline A$. Therefore, $f(k')$ must belong to $A \setminus \interior(A) = \iboundary(A)$.
% \end{proof}


% \begin{todo}
%  \cite{Gal03} defines \emph{linked} points in a quasi-discrete closure space as those points that are connected by a \emph{finite} path. However, I think the definition should take into account also infinite structures (what about Lemma 13 for the quasi-discrete space associated to $(\mathbb{Q},\leq)$?).
% \end{todo}

% 
% \begin{lemma}\label{lem:closure-path-is-graph-path}
%  In a quasi-discrete closure space $(X,\closure_R)$, a path in the sense of \autoref{def:path} is a path over the graph of $R$, in the traditional graph-theoretical sense. More formally, there is a one-to-one correspondence between closure-based paths from $x$ to $y$, and sequences of points $\{x_i\}_\{i \in [0,\ldots,n]\}$, with $n\geq 0$ a natural number, such that $x_0 = x$, $x_n = y$, and $\forall i \in [0,\ldots,n-1] . (x_i,x_{i+1}) \in R$.
% \end{lemma}
% 
% \begin{proof}(of \autoref{lem:closure-path-is-graph-path}
%  Consider a path $f$ in the sense of \autoref{def:path}. 
% \end{proof}





==> design-until.tex <==
\section{The design of a spatial \emph{until} operator}
\label{sec:issues}

This paper is about spatial logics in closure spaces. Before introducing the complete framework, in this section, we discuss the design of an \emph{until operator}, that is, a binary logical connective of the form $\phi \until \psi$, with a natural intended meaning, that we state as a design principle.

\begin{principle}\label{pri:until}
We aim at defining a binary spatial logical operator $\until$, interpreted on points of a closure space. The basic idea is that point $x$ satisfies $\phi \until \psi$ whenever it is included in an area $A$ satisfying $\phi$, and there is ``no way out'' from $A$ unless passing trough an area $B$ that satisfies $\psi$.
\end{principle}

To turn this principle into a mathematical definition, one should clarify the meaning of the words \emph{area}, \emph{included}, \emph{passing}, in the context of closure spaces. The variables are many. Consider the area $A$. Is it possible for $A$ to be the singleton $x$, or do we require that $x$ has a proper neighbourhood of points satisfying $\phi$? This is more relevant in continuous spaces, where singletons are problematic (for example, in Euclidean spaces, they have measure $0$). 
%A problem is how to clearly distinguish the outside from the inside of a boundary. We shall see that it is in general not possible to do so. 
%However, in finite spaces, it may be possible to define a set of points that are considered \emph{extremal}, so that the inside of a boundary may be told apart by observing the presence of an extremal point into a region. 
Definitions that are satisfactory in discrete spaces may have issues when switching to continuous domains, and vice-versa. We start from the topological definition of \emph{until}, and investigate the situation with respect to \autoref{pri:until}. For this, we need to define a \emph{model}, providing a context of evaluation for the satisfaction relation, as in $\model, x \models \phi \until \psi$.

\begin{definition}\label{def:model}
 A \emph{closure model} is a pair $\model = ((X,\closure),\eval)$ consisting of a closure space $(X,\closure)$ and a valuation $\eval : \props \to 2^X$, assigning to each proposition letter the set of points where the proposition holds.
\end{definition}
 
 When $(X,\closure)$ is the interpretation of a topological space as a closure space, we call $\model$ a \emph{topological model}, in line with the definition used in \cite{vBB07}, and \cite{A02}. Therein, the \emph{topological until} operator is presented. We recall it below.

\begin{definition}\label{def:until-t}
 The \emph{topological until} operator $\until_T$ is interpreted in a topological model $\model$ as $\model,x \models \phi \until_T \psi \iff \exists A$ open $ . x \in A \land \forall y \in A . \model, y \models \phi \land \forall z \in \boundary(A) . \model, z \models \psi$. 
\end{definition}

The intuition behind this definition is that one seeks for an area $A$ (which, topologically speaking, could sensibly be an open set) where $\phi$ holds, and that is completely surrounded by points where $\psi$ holds. First, we report about a well-known problem of notions such as ``inside'' and ``outside'' in topology.

\begin{issue}\label{iss:until-t-outside}
\autoref{def:until-t} does not distinguish the inside from the outside of a boundary. Let $C = \{ (x,y) \in \reals^2 \mid x^2 + y^2 = 1 \}$ be the circumference of radius $1$ in $\reals^2$, $x$ a point inside of $C$ (e.g., $(0,0)$), $y$ a point outside of $C$ (e.g., $(2,2)$). Consider a topological model based on $\reals^2$ (with the Euclidean topology) such that $\eval(p) = \reals^2 \setminus C$ and $\eval(q) = C$. Then we have $x \models p \until_T q$. This is in accordance to our stated requirements. But $y$ satisfies $p \until_T q$ as well, as can be easily checked, by choosing as the set $A$ \emph{all} the points outside of $C$.
\end{issue}

\autoref{iss:until-t-outside} is a well-known subject in topology, stemming from the statement of \emph{Jordan's theorem}: the complement of a closed curve $C$ in $\reals^2$ consists of exactly two connected components $A$ and $A'$. The statement of the theorem does not make a distinction between $A$ and $A'$. In a general topological space, it is not actually possible to make such a distinction (think of a closed curve on the surface of a sphere). In Euclidean spaces, to address this, one may resort to \emph{homotopy} \cite{Whi78}. Investigating an appropriate notion of homotopy in closure spaces is not a trivial task. For example, in graphs, it is always possible to rearrange nodes, so notions of ``inside'' and ``outside'' can not be simply translated from Euclidean spaces. 

In this work, we will seek for a more pragmatic approach. We shall assume that, on a by-need basis, one may make use of predicates denoting ``extremal points'' that should not be reachable by any point satisfying an until formula. This is reasonable in finite models as they typically are submodels of some infinite model, where a boundary has been used to delineate the ``end of the world''. In this situation, let $e$ be a proposition letter denoting the extremal points; then the formula $(\phi \land \lnot e) \until_T \phi$ distinguishes points that are ``inside'' $\psi$ (and satisfy $\phi$), from points that are ``outside'' of it. Once this is established, we ought to seek for a definition which is apt to closure spaces.

\begin{issue}\label{iss:open-boundary}
\autoref{def:until-t} can not be translated directly to closure spaces, even if all the used topological notions have a counterpart in the more general setting. Open sets in closure spaces are often too coarse (see \autoref{rem:open-sets-coarse}). Moreover, the usage of $\boundary$ in \autoref{def:until-t} is not satisfactory either. By \autoref{pro:boundary-properties} we have $\boundary(A) = \cboundary(A) \cup \iboundary(A)$. Let us look at the closure space $(\ints^2,\closure)$ induced by the graph with nodes in $\ints^2$ and edges linking each point $(x,y)$ to its four neighbours\footnote{In the literature, such space is sometimes referred to as the \emph{digital plane}; however, the same term may also denote $\ints^2$ equipped with different notions of neighbourhood.} $(x-1,y),(x+1,y),(x,y-1),(x,y+1)$. Consider a rectangle $A$ such that all points in $A$ satisfy $\phi$ and all points in $\iboundary(A)$ satisfy $\psi$, whereas all points in $\overline A$ do not satisfy $\phi$ or $\psi$. Then each point in $\interior(A)$ is enclosed in the region delimited by $\psi$, thus satisfying $\phi \until \psi$ according to \autoref{pri:until}. However, not all points in $\boundary(A)$ satisfy $\psi$, as $\psi$ does not hold in $\cboundary(A)$ .
\end{issue}

By \autoref{iss:open-boundary}, we could chose either $\iboundary$ or $\cboundary$ to play the same role as $\boundary$. In the first case, we shall seek for a set $A$ such that all points in its \emph{interior} satisfy $\phi$, and all the points in $\iboundary(A)$ satisfy $\psi$. In the second case, we shall instead require that $\phi$ is satisfied by \emph{all} the points of $A$, and that in $\cboundary(A)$, $\psi$ holds. This is to ensure that there are no ``gaps'' between $\phi$ and $\psi$. The definition using $\iboundary$ presents an additional problem.

%Additionally, we shall require that the chosen boundary is not empty. This is a design choice, that avoids the following situation: if the boundary satisfying $\psi$ is allowed to be empty, consider a space where all points satisfy $\phi$ and no point satisfies $\psi$; then points in the set $X$ of all points of the space would satisfy $\phi \until \psi$ by the fact that $\interior(X) =  \closure(X) = X$, thus $\boundary(X) = \iboundary(X) = \cboundary(X) = \emptyset$.  


% 
% \begin{definition}\label{def:until-c-iboundary}
%  The operator $\until_{C^-}$ is interpreted as $\model,x \models \phi \until_{C^-} \psi \iff \exists A . x \in \interior(A) \land \forall y \in \interior(A) . \model, y \models \phi \land \forall z \in \iboundary(A) . \model, z \models \psi \land \iboundary(A) \neq \emptyset$.
% \end{definition}


\begin{issue}\label{iss:cboundary-better}
 Consider the closure space $(\ints^2,\closure)$ described in \autoref{iss:open-boundary}. Consider the ``cross'' $H = \{ (-1,0), (0,0), (1,0), (0,-1), (0,1) \}$ where point $x = (0,0)$ satisfies $\phi$ and the remaining points satisfy $\psi$. Let $A = H$. Then $\interior(A) = \{ x\}$ satisfies $\phi$ and $\iboundary(A)$ satisfies $\psi$, agreeing with our intuition. However, if we restrict the space to $(H,\closure)$ (see \autoref{def:subspace}), then $A$ is the set of all points, thus $\interior(A) = A$ and $\iboundary(A) = \emptyset$. Therefore, not all points of $\interior(A)$ satisfy $\phi$. A quick analysis of all the possible choices for $A$ shows that, in this case, it is impossible to find $A$ such that $\phi$ holds in $\interior(A)$ and $\psi$ holds in $\iboundary(A)$. 
\end{issue}

Furthermore, in closure spaces $(X,\closure_R)$ derived from a non-symmetric relation $R$, $\iboundary(A)$ is the set of points that have \emph{incoming} edges from $\overline A$ (see \autoref{pro:interior-boundary-in-quasi-discrete}). As in \autoref{pri:until} we mention the idea of having ``no way \emph{out}'' of $A$, it intuitively makes sense to consider $\cboundary(A)$ instead. In \autoref{sec:dsl} and \autoref{sec:discrete-examples}, we shall see how all these observations converge to a definition which behaves according to \autoref{pri:until} over discrete structures. Continuous structures are far more complex to study; a discussion is provided in \autoref{sec:discussion}.





==> figures/contaminated-area-1-out.tex <==
\begin{tikzpicture}{}
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (6*0.8,7*0.8) (nodeX6Y7) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (7*0.8,7*0.8) (nodeX7Y7) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,7*0.8) (nodeX3Y7) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (4*0.8,7*0.8) (nodeX4Y7) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (8*0.8,7*0.8) (nodeX8Y7) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (8*0.8,6*0.8) (nodeX8Y6) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (7*0.8,6*0.8) (nodeX7Y6) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (5*0.8,7*0.8) (nodeX5Y7) {};
  \node [circle,draw=blue!50,fill=blue!20,thick,inner sep=0pt,minimum size=4mm] at (6*0.8,6*0.8) (nodeX6Y6) {};
  \node [circle,draw=cyan!50,fill=cyan!20,thick,inner sep=0pt,minimum size=4mm] at (5*0.8,6*0.8) (nodeX5Y6) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,6*0.8) (nodeX3Y6) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (4*0.8,6*0.8) (nodeX4Y6) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (6*0.8,5*0.8) (nodeX6Y5) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (7*0.8,5*0.8) (nodeX7Y5) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (4*0.8,5*0.8) (nodeX4Y5) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (8*0.8,5*0.8) (nodeX8Y5) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (6*0.8,4*0.8) (nodeX6Y4) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (7*0.8,4*0.8) (nodeX7Y4) {};
  \node [circle,draw=blue!50,fill=blue!20,thick,inner sep=0pt,minimum size=4mm] at (5*0.8,5*0.8) (nodeX5Y5) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,5*0.8) (nodeX3Y5) {};
  \node [circle,draw=blue!50,fill=blue!20,thick,inner sep=0pt,minimum size=4mm] at (4*0.8,4*0.8) (nodeX4Y4) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (8*0.8,4*0.8) (nodeX8Y4) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (8*0.8,3*0.8) (nodeX8Y3) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (6*0.8,3*0.8) (nodeX6Y3) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (7*0.8,3*0.8) (nodeX7Y3) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (5*0.8,4*0.8) (nodeX5Y4) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (5*0.8,3*0.8) (nodeX5Y3) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,4*0.8) (nodeX3Y4) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (4*0.8,3*0.8) (nodeX4Y3) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (1*0.8,3*0.8) (nodeX1Y3) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (2*0.8,3*0.8) (nodeX2Y3) {};
  \node [circle,draw=blue!50,fill=blue!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,3*0.8) (nodeX3Y3) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (1*0.8,2*0.8) (nodeX1Y2) {};
  \node [circle,draw=blue!50,fill=blue!20,thick,inner sep=0pt,minimum size=4mm] at (2*0.8,2*0.8) (nodeX2Y2) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,2*0.8) (nodeX3Y2) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,1*0.8) (nodeX3Y1) {};
  \node [circle,draw=blue!50,fill=blue!20,thick,inner sep=0pt,minimum size=4mm] at (1*0.8,1*0.8) (nodeX1Y1) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (2*0.8,1*0.8) (nodeX2Y1) {};

  \draw[->] (nodeX1Y1) -- (nodeX2Y1);
  \draw[->] (nodeX2Y1) -- (nodeX3Y1);
  \draw[->] (nodeX2Y1) -- (nodeX1Y1);
  \draw[->] (nodeX3Y1) -- (nodeX2Y1);
  \draw[->] (nodeX3Y1) -- (nodeX3Y2);
  \draw[->] (nodeX1Y2) -- (nodeX2Y2);
  \draw[->] (nodeX2Y2) -- (nodeX3Y2);
  \draw[->] (nodeX2Y2) -- (nodeX1Y2);
  \draw[->] (nodeX3Y2) -- (nodeX2Y2);
  \draw[->] (nodeX3Y2) -- (nodeX3Y3);
  \draw[->] (nodeX1Y3) -- (nodeX2Y3);
  \draw[->] (nodeX2Y3) -- (nodeX3Y3);
  \draw[->] (nodeX2Y3) -- (nodeX1Y3);
  \draw[->] (nodeX3Y3) -- (nodeX4Y3);
  \draw[->] (nodeX3Y3) -- (nodeX2Y3);
  \draw[->] (nodeX3Y3) -- (nodeX3Y4);
  \draw[->] (nodeX4Y3) -- (nodeX5Y3);
  \draw[->] (nodeX4Y3) -- (nodeX3Y3);
  \draw[->] (nodeX5Y3) -- (nodeX5Y4);
  \draw[->] (nodeX6Y3) -- (nodeX7Y3);
  \draw[->] (nodeX6Y3) -- (nodeX5Y3);
  \draw[->] (nodeX7Y3) -- (nodeX8Y3);
  \draw[->] (nodeX7Y3) -- (nodeX6Y3);
  \draw[->] (nodeX8Y3) -- (nodeX7Y3);
  \draw[->] (nodeX8Y3) -- (nodeX8Y4);
  \draw[->] (nodeX3Y4) -- (nodeX4Y4);
  \draw[->] (nodeX3Y4) -- (nodeX3Y5);
  \draw[->] (nodeX4Y4) -- (nodeX5Y4);
  \draw[->] (nodeX4Y4) -- (nodeX3Y4);
  \draw[->] (nodeX5Y4) -- (nodeX5Y5);
  \draw[->] (nodeX6Y4) -- (nodeX7Y4);
  \draw[->] (nodeX6Y4) -- (nodeX5Y4);
  \draw[->] (nodeX7Y4) -- (nodeX8Y4);
  \draw[->] (nodeX7Y4) -- (nodeX6Y4);
  \draw[->] (nodeX8Y4) -- (nodeX7Y4);
  \draw[->] (nodeX8Y4) -- (nodeX8Y5);
  \draw[->] (nodeX3Y5) -- (nodeX4Y5);
  \draw[->] (nodeX4Y5) -- (nodeX5Y5);
  \draw[->] (nodeX4Y5) -- (nodeX3Y5);
  \draw[->] (nodeX6Y5) -- (nodeX7Y5);
  \draw[->] (nodeX6Y5) -- (nodeX5Y5);
  \draw[->] (nodeX7Y5) -- (nodeX8Y5);
  \draw[->] (nodeX7Y5) -- (nodeX6Y5);
  \draw[->] (nodeX8Y5) -- (nodeX7Y5);
  \draw[->] (nodeX3Y6) -- (nodeX4Y6);
  \draw[->] (nodeX4Y6) -- (nodeX5Y6);
  \draw[->] (nodeX4Y6) -- (nodeX3Y6);
  \draw[->] (nodeX5Y6) -- (nodeX6Y6);
  \draw[->] (nodeX5Y6) -- (nodeX5Y5);
  \draw[->] (nodeX5Y6) -- (nodeX5Y7);
  \draw[->] (nodeX6Y6) -- (nodeX7Y6);
  \draw[->] (nodeX7Y6) -- (nodeX8Y6);
  \draw[->] (nodeX7Y6) -- (nodeX6Y6);
  \draw[->] (nodeX8Y6) -- (nodeX7Y6);
  \draw[->] (nodeX8Y6) -- (nodeX8Y7);
  \draw[->] (nodeX3Y7) -- (nodeX4Y7);
  \draw[->] (nodeX4Y7) -- (nodeX5Y7);
  \draw[->] (nodeX4Y7) -- (nodeX3Y7);
  \draw[->] (nodeX6Y7) -- (nodeX7Y7);
  \draw[->] (nodeX6Y7) -- (nodeX5Y7);
  \draw[->] (nodeX7Y7) -- (nodeX8Y7);
  \draw[->] (nodeX7Y7) -- (nodeX6Y7);
  \draw[->] (nodeX8Y7) -- (nodeX7Y7);
\end{tikzpicture}


==> figures/contaminated-area-2-out.tex <==
\begin{tikzpicture}{}
  \node [circle,draw=orange!50,fill=orange!20,thick,inner sep=0pt,minimum size=4mm] at (6*0.8,7*0.8) (nodeX6Y7) {};
  \node [circle,draw=orange!50,fill=orange!20,thick,inner sep=0pt,minimum size=4mm] at (7*0.8,7*0.8) (nodeX7Y7) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,7*0.8) (nodeX3Y7) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (4*0.8,7*0.8) (nodeX4Y7) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (8*0.8,7*0.8) (nodeX8Y7) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (8*0.8,6*0.8) (nodeX8Y6) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (7*0.8,6*0.8) (nodeX7Y6) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (5*0.8,7*0.8) (nodeX5Y7) {};
  \node [circle,draw=blue!50,fill=blue!20,thick,inner sep=0pt,minimum size=4mm] at (6*0.8,6*0.8) (nodeX6Y6) {};
  \node [circle,draw=cyan!50,fill=cyan!20,thick,inner sep=0pt,minimum size=4mm] at (5*0.8,6*0.8) (nodeX5Y6) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,6*0.8) (nodeX3Y6) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (4*0.8,6*0.8) (nodeX4Y6) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (6*0.8,5*0.8) (nodeX6Y5) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (7*0.8,5*0.8) (nodeX7Y5) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (4*0.8,5*0.8) (nodeX4Y5) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (8*0.8,5*0.8) (nodeX8Y5) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (6*0.8,4*0.8) (nodeX6Y4) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (7*0.8,4*0.8) (nodeX7Y4) {};
  \node [circle,draw=blue!50,fill=blue!20,thick,inner sep=0pt,minimum size=4mm] at (5*0.8,5*0.8) (nodeX5Y5) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,5*0.8) (nodeX3Y5) {};
  \node [circle,draw=blue!50,fill=blue!20,thick,inner sep=0pt,minimum size=4mm] at (4*0.8,4*0.8) (nodeX4Y4) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (8*0.8,4*0.8) (nodeX8Y4) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (8*0.8,3*0.8) (nodeX8Y3) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (6*0.8,3*0.8) (nodeX6Y3) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (7*0.8,3*0.8) (nodeX7Y3) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (5*0.8,4*0.8) (nodeX5Y4) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (5*0.8,3*0.8) (nodeX5Y3) {};
  \node [circle,draw=orange!50,fill=orange!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,4*0.8) (nodeX3Y4) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (4*0.8,3*0.8) (nodeX4Y3) {};
  \node [circle,draw=orange!50,fill=orange!20,thick,inner sep=0pt,minimum size=4mm] at (1*0.8,3*0.8) (nodeX1Y3) {};
  \node [circle,draw=orange!50,fill=orange!20,thick,inner sep=0pt,minimum size=4mm] at (2*0.8,3*0.8) (nodeX2Y3) {};
  \node [circle,draw=blue!50,fill=blue!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,3*0.8) (nodeX3Y3) {};
  \node [circle,draw=orange!50,fill=orange!20,thick,inner sep=0pt,minimum size=4mm] at (1*0.8,2*0.8) (nodeX1Y2) {};
  \node [circle,draw=blue!50,fill=blue!20,thick,inner sep=0pt,minimum size=4mm] at (2*0.8,2*0.8) (nodeX2Y2) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,2*0.8) (nodeX3Y2) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,1*0.8) (nodeX3Y1) {};
  \node [circle,draw=blue!50,fill=blue!20,thick,inner sep=0pt,minimum size=4mm] at (1*0.8,1*0.8) (nodeX1Y1) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (2*0.8,1*0.8) (nodeX2Y1) {};

  \draw[->] (nodeX1Y1) -- (nodeX2Y1);
  \draw[->] (nodeX2Y1) -- (nodeX3Y1);
  \draw[->] (nodeX2Y1) -- (nodeX1Y1);
  \draw[->] (nodeX3Y1) -- (nodeX2Y1);
  \draw[->] (nodeX3Y1) -- (nodeX3Y2);
  \draw[->] (nodeX1Y2) -- (nodeX2Y2);
  \draw[->] (nodeX2Y2) -- (nodeX3Y2);
  \draw[->] (nodeX2Y2) -- (nodeX1Y2);
  \draw[->] (nodeX3Y2) -- (nodeX2Y2);
  \draw[->] (nodeX3Y2) -- (nodeX3Y3);
  \draw[->] (nodeX1Y3) -- (nodeX2Y3);
  \draw[->] (nodeX2Y3) -- (nodeX3Y3);
  \draw[->] (nodeX2Y3) -- (nodeX1Y3);
  \draw[->] (nodeX3Y3) -- (nodeX4Y3);
  \draw[->] (nodeX3Y3) -- (nodeX2Y3);
  \draw[->] (nodeX3Y3) -- (nodeX3Y4);
  \draw[->] (nodeX4Y3) -- (nodeX5Y3);
  \draw[->] (nodeX4Y3) -- (nodeX3Y3);
  \draw[->] (nodeX5Y3) -- (nodeX5Y4);
  \draw[->] (nodeX6Y3) -- (nodeX7Y3);
  \draw[->] (nodeX6Y3) -- (nodeX5Y3);
  \draw[->] (nodeX7Y3) -- (nodeX8Y3);
  \draw[->] (nodeX7Y3) -- (nodeX6Y3);
  \draw[->] (nodeX8Y3) -- (nodeX7Y3);
  \draw[->] (nodeX8Y3) -- (nodeX8Y4);
  \draw[->] (nodeX3Y4) -- (nodeX4Y4);
  \draw[->] (nodeX3Y4) -- (nodeX3Y5);
  \draw[->] (nodeX4Y4) -- (nodeX5Y4);
  \draw[->] (nodeX4Y4) -- (nodeX3Y4);
  \draw[->] (nodeX5Y4) -- (nodeX5Y5);
  \draw[->] (nodeX6Y4) -- (nodeX7Y4);
  \draw[->] (nodeX6Y4) -- (nodeX5Y4);
  \draw[->] (nodeX7Y4) -- (nodeX8Y4);
  \draw[->] (nodeX7Y4) -- (nodeX6Y4);
  \draw[->] (nodeX8Y4) -- (nodeX7Y4);
  \draw[->] (nodeX8Y4) -- (nodeX8Y5);
  \draw[->] (nodeX3Y5) -- (nodeX4Y5);
  \draw[->] (nodeX4Y5) -- (nodeX5Y5);
  \draw[->] (nodeX4Y5) -- (nodeX3Y5);
  \draw[->] (nodeX6Y5) -- (nodeX7Y5);
  \draw[->] (nodeX6Y5) -- (nodeX5Y5);
  \draw[->] (nodeX7Y5) -- (nodeX8Y5);
  \draw[->] (nodeX7Y5) -- (nodeX6Y5);
  \draw[->] (nodeX8Y5) -- (nodeX7Y5);
  \draw[->] (nodeX3Y6) -- (nodeX4Y6);
  \draw[->] (nodeX4Y6) -- (nodeX5Y6);
  \draw[->] (nodeX4Y6) -- (nodeX3Y6);
  \draw[->] (nodeX5Y6) -- (nodeX6Y6);
  \draw[->] (nodeX5Y6) -- (nodeX5Y5);
  \draw[->] (nodeX5Y6) -- (nodeX5Y7);
  \draw[->] (nodeX6Y6) -- (nodeX7Y6);
  \draw[->] (nodeX7Y6) -- (nodeX8Y6);
  \draw[->] (nodeX7Y6) -- (nodeX6Y6);
  \draw[->] (nodeX8Y6) -- (nodeX7Y6);
  \draw[->] (nodeX8Y6) -- (nodeX8Y7);
  \draw[->] (nodeX3Y7) -- (nodeX4Y7);
  \draw[->] (nodeX4Y7) -- (nodeX5Y7);
  \draw[->] (nodeX4Y7) -- (nodeX3Y7);
  \draw[->] (nodeX6Y7) -- (nodeX7Y7);
  \draw[->] (nodeX6Y7) -- (nodeX5Y7);
  \draw[->] (nodeX7Y7) -- (nodeX8Y7);
  \draw[->] (nodeX7Y7) -- (nodeX6Y7);
  \draw[->] (nodeX8Y7) -- (nodeX7Y7);
\end{tikzpicture}


==> figures/contaminated-area-3-out.tex <==
\begin{tikzpicture}{}
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (6*0.8,7*0.8) (nodeX6Y7) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (7*0.8,7*0.8) (nodeX7Y7) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,7*0.8) (nodeX3Y7) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (4*0.8,7*0.8) (nodeX4Y7) {};
  \node [circle,draw=orange!50,fill=orange!20,thick,inner sep=0pt,minimum size=4mm] at (8*0.8,7*0.8) (nodeX8Y7) {};
  \node [circle,draw=orange!50,fill=orange!20,thick,inner sep=0pt,minimum size=4mm] at (8*0.8,6*0.8) (nodeX8Y6) {};
  \node [circle,draw=orange!50,fill=orange!20,thick,inner sep=0pt,minimum size=4mm] at (7*0.8,6*0.8) (nodeX7Y6) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (5*0.8,7*0.8) (nodeX5Y7) {};
  \node [circle,draw=blue!50,fill=blue!20,thick,inner sep=0pt,minimum size=4mm] at (6*0.8,6*0.8) (nodeX6Y6) {};
  \node [circle,draw=cyan!50,fill=cyan!20,thick,inner sep=0pt,minimum size=4mm] at (5*0.8,6*0.8) (nodeX5Y6) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,6*0.8) (nodeX3Y6) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (4*0.8,6*0.8) (nodeX4Y6) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (6*0.8,5*0.8) (nodeX6Y5) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (7*0.8,5*0.8) (nodeX7Y5) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (4*0.8,5*0.8) (nodeX4Y5) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (8*0.8,5*0.8) (nodeX8Y5) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (6*0.8,4*0.8) (nodeX6Y4) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (7*0.8,4*0.8) (nodeX7Y4) {};
  \node [circle,draw=blue!50,fill=blue!20,thick,inner sep=0pt,minimum size=4mm] at (5*0.8,5*0.8) (nodeX5Y5) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,5*0.8) (nodeX3Y5) {};
  \node [circle,draw=blue!50,fill=blue!20,thick,inner sep=0pt,minimum size=4mm] at (4*0.8,4*0.8) (nodeX4Y4) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (8*0.8,4*0.8) (nodeX8Y4) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (8*0.8,3*0.8) (nodeX8Y3) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (6*0.8,3*0.8) (nodeX6Y3) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (7*0.8,3*0.8) (nodeX7Y3) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (5*0.8,4*0.8) (nodeX5Y4) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (5*0.8,3*0.8) (nodeX5Y3) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,4*0.8) (nodeX3Y4) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (4*0.8,3*0.8) (nodeX4Y3) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (1*0.8,3*0.8) (nodeX1Y3) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (2*0.8,3*0.8) (nodeX2Y3) {};
  \node [circle,draw=blue!50,fill=blue!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,3*0.8) (nodeX3Y3) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (1*0.8,2*0.8) (nodeX1Y2) {};
  \node [circle,draw=blue!50,fill=blue!20,thick,inner sep=0pt,minimum size=4mm] at (2*0.8,2*0.8) (nodeX2Y2) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,2*0.8) (nodeX3Y2) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,1*0.8) (nodeX3Y1) {};
  \node [circle,draw=blue!50,fill=blue!20,thick,inner sep=0pt,minimum size=4mm] at (1*0.8,1*0.8) (nodeX1Y1) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (2*0.8,1*0.8) (nodeX2Y1) {};

  \draw[->] (nodeX1Y1) -- (nodeX2Y1);
  \draw[->] (nodeX2Y1) -- (nodeX3Y1);
  \draw[->] (nodeX2Y1) -- (nodeX1Y1);
  \draw[->] (nodeX3Y1) -- (nodeX2Y1);
  \draw[->] (nodeX3Y1) -- (nodeX3Y2);
  \draw[->] (nodeX1Y2) -- (nodeX2Y2);
  \draw[->] (nodeX2Y2) -- (nodeX3Y2);
  \draw[->] (nodeX2Y2) -- (nodeX1Y2);
  \draw[->] (nodeX3Y2) -- (nodeX2Y2);
  \draw[->] (nodeX3Y2) -- (nodeX3Y3);
  \draw[->] (nodeX1Y3) -- (nodeX2Y3);
  \draw[->] (nodeX2Y3) -- (nodeX3Y3);
  \draw[->] (nodeX2Y3) -- (nodeX1Y3);
  \draw[->] (nodeX3Y3) -- (nodeX4Y3);
  \draw[->] (nodeX3Y3) -- (nodeX2Y3);
  \draw[->] (nodeX3Y3) -- (nodeX3Y4);
  \draw[->] (nodeX4Y3) -- (nodeX5Y3);
  \draw[->] (nodeX4Y3) -- (nodeX3Y3);
  \draw[->] (nodeX5Y3) -- (nodeX5Y4);
  \draw[->] (nodeX6Y3) -- (nodeX7Y3);
  \draw[->] (nodeX6Y3) -- (nodeX5Y3);
  \draw[->] (nodeX7Y3) -- (nodeX8Y3);
  \draw[->] (nodeX7Y3) -- (nodeX6Y3);
  \draw[->] (nodeX8Y3) -- (nodeX7Y3);
  \draw[->] (nodeX8Y3) -- (nodeX8Y4);
  \draw[->] (nodeX3Y4) -- (nodeX4Y4);
  \draw[->] (nodeX3Y4) -- (nodeX3Y5);
  \draw[->] (nodeX4Y4) -- (nodeX5Y4);
  \draw[->] (nodeX4Y4) -- (nodeX3Y4);
  \draw[->] (nodeX5Y4) -- (nodeX5Y5);
  \draw[->] (nodeX6Y4) -- (nodeX7Y4);
  \draw[->] (nodeX6Y4) -- (nodeX5Y4);
  \draw[->] (nodeX7Y4) -- (nodeX8Y4);
  \draw[->] (nodeX7Y4) -- (nodeX6Y4);
  \draw[->] (nodeX8Y4) -- (nodeX7Y4);
  \draw[->] (nodeX8Y4) -- (nodeX8Y5);
  \draw[->] (nodeX3Y5) -- (nodeX4Y5);
  \draw[->] (nodeX4Y5) -- (nodeX5Y5);
  \draw[->] (nodeX4Y5) -- (nodeX3Y5);
  \draw[->] (nodeX6Y5) -- (nodeX7Y5);
  \draw[->] (nodeX6Y5) -- (nodeX5Y5);
  \draw[->] (nodeX7Y5) -- (nodeX8Y5);
  \draw[->] (nodeX7Y5) -- (nodeX6Y5);
  \draw[->] (nodeX8Y5) -- (nodeX7Y5);
  \draw[->] (nodeX3Y6) -- (nodeX4Y6);
  \draw[->] (nodeX4Y6) -- (nodeX5Y6);
  \draw[->] (nodeX4Y6) -- (nodeX3Y6);
  \draw[->] (nodeX5Y6) -- (nodeX6Y6);
  \draw[->] (nodeX5Y6) -- (nodeX5Y5);
  \draw[->] (nodeX5Y6) -- (nodeX5Y7);
  \draw[->] (nodeX6Y6) -- (nodeX7Y6);
  \draw[->] (nodeX7Y6) -- (nodeX8Y6);
  \draw[->] (nodeX7Y6) -- (nodeX6Y6);
  \draw[->] (nodeX8Y6) -- (nodeX7Y6);
  \draw[->] (nodeX8Y6) -- (nodeX8Y7);
  \draw[->] (nodeX3Y7) -- (nodeX4Y7);
  \draw[->] (nodeX4Y7) -- (nodeX5Y7);
  \draw[->] (nodeX4Y7) -- (nodeX3Y7);
  \draw[->] (nodeX6Y7) -- (nodeX7Y7);
  \draw[->] (nodeX6Y7) -- (nodeX5Y7);
  \draw[->] (nodeX7Y7) -- (nodeX8Y7);
  \draw[->] (nodeX7Y7) -- (nodeX6Y7);
  \draw[->] (nodeX8Y7) -- (nodeX7Y7);
\end{tikzpicture}


==> figures/contaminated-area-4-out.tex <==
\begin{tikzpicture}{}
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (6*0.8,7*0.8) (nodeX6Y7) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (7*0.8,7*0.8) (nodeX7Y7) {};
  \node [circle,draw=orange!50,fill=orange!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,7*0.8) (nodeX3Y7) {};
  \node [circle,draw=orange!50,fill=orange!20,thick,inner sep=0pt,minimum size=4mm] at (4*0.8,7*0.8) (nodeX4Y7) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (8*0.8,7*0.8) (nodeX8Y7) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (8*0.8,6*0.8) (nodeX8Y6) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (7*0.8,6*0.8) (nodeX7Y6) {};
  \node [circle,draw=orange!50,fill=orange!20,thick,inner sep=0pt,minimum size=4mm] at (5*0.8,7*0.8) (nodeX5Y7) {};
  \node [circle,draw=blue!50,fill=blue!20,thick,inner sep=0pt,minimum size=4mm] at (6*0.8,6*0.8) (nodeX6Y6) {};
  \node [circle,draw=cyan!50,fill=cyan!20,thick,inner sep=0pt,minimum size=4mm] at (5*0.8,6*0.8) (nodeX5Y6) {};
  \node [circle,draw=orange!50,fill=orange!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,6*0.8) (nodeX3Y6) {};
  \node [circle,draw=orange!50,fill=orange!20,thick,inner sep=0pt,minimum size=4mm] at (4*0.8,6*0.8) (nodeX4Y6) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (6*0.8,5*0.8) (nodeX6Y5) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (7*0.8,5*0.8) (nodeX7Y5) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (4*0.8,5*0.8) (nodeX4Y5) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (8*0.8,5*0.8) (nodeX8Y5) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (6*0.8,4*0.8) (nodeX6Y4) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (7*0.8,4*0.8) (nodeX7Y4) {};
  \node [circle,draw=blue!50,fill=blue!20,thick,inner sep=0pt,minimum size=4mm] at (5*0.8,5*0.8) (nodeX5Y5) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,5*0.8) (nodeX3Y5) {};
  \node [circle,draw=blue!50,fill=blue!20,thick,inner sep=0pt,minimum size=4mm] at (4*0.8,4*0.8) (nodeX4Y4) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (8*0.8,4*0.8) (nodeX8Y4) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (8*0.8,3*0.8) (nodeX8Y3) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (6*0.8,3*0.8) (nodeX6Y3) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (7*0.8,3*0.8) (nodeX7Y3) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (5*0.8,4*0.8) (nodeX5Y4) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (5*0.8,3*0.8) (nodeX5Y3) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,4*0.8) (nodeX3Y4) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (4*0.8,3*0.8) (nodeX4Y3) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (1*0.8,3*0.8) (nodeX1Y3) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (2*0.8,3*0.8) (nodeX2Y3) {};
  \node [circle,draw=blue!50,fill=blue!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,3*0.8) (nodeX3Y3) {};
  \node [circle,draw=green!50,fill=green!20,thick,inner sep=0pt,minimum size=4mm] at (1*0.8,2*0.8) (nodeX1Y2) {};
  \node [circle,draw=blue!50,fill=blue!20,thick,inner sep=0pt,minimum size=4mm] at (2*0.8,2*0.8) (nodeX2Y2) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,2*0.8) (nodeX3Y2) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (3*0.8,1*0.8) (nodeX3Y1) {};
  \node [circle,draw=blue!50,fill=blue!20,thick,inner sep=0pt,minimum size=4mm] at (1*0.8,1*0.8) (nodeX1Y1) {};
  \node [circle,draw=red!50,fill=red!20,thick,inner sep=0pt,minimum size=4mm] at (2*0.8,1*0.8) (nodeX2Y1) {};

  \draw[->] (nodeX1Y1) -- (nodeX2Y1);
  \draw[->] (nodeX2Y1) -- (nodeX3Y1);
  \draw[->] (nodeX2Y1) -- (nodeX1Y1);
  \draw[->] (nodeX3Y1) -- (nodeX2Y1);
  \draw[->] (nodeX3Y1) -- (nodeX3Y2);
  \draw[->] (nodeX1Y2) -- (nodeX2Y2);
  \draw[->] (nodeX2Y2) -- (nodeX3Y2);
  \draw[->] (nodeX2Y2) -- (nodeX1Y2);
  \draw[->] (nodeX3Y2) -- (nodeX2Y2);
  \draw[->] (nodeX3Y2) -- (nodeX3Y3);
  \draw[->] (nodeX1Y3) -- (nodeX2Y3);
  \draw[->] (nodeX2Y3) -- (nodeX3Y3);
  \draw[->] (nodeX2Y3) -- (nodeX1Y3);
  \draw[->] (nodeX3Y3) -- (nodeX4Y3);
  \draw[->] (nodeX3Y3) -- (nodeX2Y3);
  \draw[->] (nodeX3Y3) -- (nodeX3Y4);
  \draw[->] (nodeX4Y3) -- (nodeX5Y3);
  \draw[->] (nodeX4Y3) -- (nodeX3Y3);
  \draw[->] (nodeX5Y3) -- (nodeX5Y4);
  \draw[->] (nodeX6Y3) -- (nodeX7Y3);
  \draw[->] (nodeX6Y3) -- (nodeX5Y3);
  \draw[->] (nodeX7Y3) -- (nodeX8Y3);
  \draw[->] (nodeX7Y3) -- (nodeX6Y3);
  \draw[->] (nodeX8Y3) -- (nodeX7Y3);
  \draw[->] (nodeX8Y3) -- (nodeX8Y4);
  \draw[->] (nodeX3Y4) -- (nodeX4Y4);
  \draw[->] (nodeX3Y4) -- (nodeX3Y5);
  \draw[->] (nodeX4Y4) -- (nodeX5Y4);
  \draw[->] (nodeX4Y4) -- (nodeX3Y4);
  \draw[->] (nodeX5Y4) -- (nodeX5Y5);
  \draw[->] (nodeX6Y4) -- (nodeX7Y4);
  \draw[->] (nodeX6Y4) -- (nodeX5Y4);
  \draw[->] (nodeX7Y4) -- (nodeX8Y4);
  \draw[->] (nodeX7Y4) -- (nodeX6Y4);
  \draw[->] (nodeX8Y4) -- (nodeX7Y4);
  \draw[->] (nodeX8Y4) -- (nodeX8Y5);
  \draw[->] (nodeX3Y5) -- (nodeX4Y5);
  \draw[->] (nodeX4Y5) -- (nodeX5Y5);
  \draw[->] (nodeX4Y5) -- (nodeX3Y5);
  \draw[->] (nodeX6Y5) -- (nodeX7Y5);
  \draw[->] (nodeX6Y5) -- (nodeX5Y5);
  \draw[->] (nodeX7Y5) -- (nodeX8Y5);
  \draw[->] (nodeX7Y5) -- (nodeX6Y5);
  \draw[->] (nodeX8Y5) -- (nodeX7Y5);
  \draw[->] (nodeX3Y6) -- (nodeX4Y6);
  \draw[->] (nodeX4Y6) -- (nodeX5Y6);
  \draw[->] (nodeX4Y6) -- (nodeX3Y6);
  \draw[->] (nodeX5Y6) -- (nodeX6Y6);
  \draw[->] (nodeX5Y6) -- (nodeX5Y5);
  \draw[->] (nodeX5Y6) -- (nodeX5Y7);
  \draw[->] (nodeX6Y6) -- (nodeX7Y6);
  \draw[->] (nodeX7Y6) -- (nodeX8Y6);
  \draw[->] (nodeX7Y6) -- (nodeX6Y6);
  \draw[->] (nodeX8Y6) -- (nodeX7Y6);
  \draw[->] (nodeX8Y6) -- (nodeX8Y7);
  \draw[->] (nodeX3Y7) -- (nodeX4Y7);
  \draw[->] (nodeX4Y7) -- (nodeX5Y7);
  \draw[->] (nodeX4Y7) -- (nodeX3Y7);
  \draw[->] (nodeX6Y7) -- (nodeX7Y7);
  \draw[->] (nodeX6Y7) -- (nodeX5Y7);
  \draw[->] (nodeX7Y7) -- (nodeX8Y7);
  \draw[->] (nodeX7Y7) -- (nodeX6Y7);
  \draw[->] (nodeX8Y7) -- (nodeX7Y7);
\end{tikzpicture}


==> more-examples.tex <==

\section{More examples}
% 
% \begin{figure}
% \begin{minipage}{.45\textwidth}
% \input{figures/maze-1-out.tex}	
% \subcaption{The model.\\~ \\~ \\}
% \end{minipage}
% \begin{minipage}{.45\textwidth}
%  \input{figures/maze-2-out.tex}
%  \subcaption{Orange: safe points from which the contaminated area may be reached without authorization.}
% \end{minipage}
% \begin{minipage}{.45\textwidth}
%  \input{figures/maze-3-out.tex}
%  \subcaption{The formula $aux$.}
% \end{minipage}
% \begin{minipage}{.45\textwidth}
%  \input{figures/maze-4-out.tex}
%  \subcaption{The formula $danger2$.}
% \end{minipage}
% %
% \begin{minipage}{\textwidth}
%  \verbatiminput{figures/maze.csmc}
% \end{minipage}
% %
% %
% \caption{Model of a contaminated building. Green nodes are safe. Red denotes contamination. Decontamination points are blue. Authorisation points are cyan. Points satisfying given formulas are in orange.}
% \end{figure}

\begin{figure}
 \begin{minipage}[t]{.45\textwidth}
    \includegraphics[width=\textwidth]{figures/maze.pdf}
    \subcaption{A maze. The green area is the exit. The blue areas are start points.}
 \end{minipage}
 \begin{minipage}[t]{.45\textwidth}
    \includegraphics[width=\textwidth]{figures/maze-out.pdf}
    \subcaption{Output from the model checker. In red, start points from which the exit can be reached. In orange, the region through which the exit can be reached from a start point. In yellow, the region from which the exit can be reached, even though there are no start points in it.}
 \end{minipage}
 \begin{minipage}{\textwidth}
  \verbatiminput{figures/maze.csmc}
  \subcaption{Input to the model checker.}
 \end{minipage}
 \caption{The model checking tool computing regions of interest in a maze.}
\end{figure}


==> temporal.tex <==
\section{Temporal aspects}\label{sec:temporal}



